ESC: Erasing Space Concept for Knowledge Deletion

As concerns regarding privacy in deep learning continue to grow, individuals are increasingly apprehensive about the potential exploitation of their personal knowledge in trained models. Despite several research efforts to address this, they often fail to consider the real-world demand from users for complete knowledge erasure. Furthermore, our investigation reveals that existing methods have a risk of leaking personal knowledge through embedding features. To address these issues, we introduce a novel concept of Knowledge Deletion (KD), an advanced task that considers both concerns, and provides an appropriate metric, named Knowledge Retention score (KR), for assessing knowledge retention in feature space. To achieve this, we propose a novel training-free erasing approach named Erasing Space Concept (ESC), which restricts the important subspace for the forgetting knowledge by eliminating the relevant activations in the feature. In addition, we suggest ESC with Training (ESC-T), which uses a learnable mask to better balance the trade-off between forgetting and preserving knowledge in KD. Our extensive experiments on various datasets and models demonstrate that our proposed methods achieve the fastest and state-of-the-art performance. Notably, our methods are applicable to diverse forgetting scenarios, such as facial domain setting, demonstrating the generalizability of our methods. The code is available at http://github.com/KU-VGI/ESC .

==> fig/fig_motivation.tex <==
\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{raw/fig_motivation2.pdf}
    \vspace{-4mm}
    \caption{Using CIFAR-10~\cite{krizhevsky2009learning} with All-CNN~\cite{springenberg2014striving}, we obtained t-SNE~\cite{van2008visualizing} results for various unlearning methods. In the retrained model, features of the forgetting class are not gathered but spread out. However, boundary shrink \cite{chen2023boundary} and LAU \cite{kim2023layer} are not changed significantly from the original model. On the other hand, our \methodname{} successfully does deep unlearning to the feature level.}
    \vspace{-5mm}
    \label{fig:motivate}
\end{figure*}

==> tab/tab_ablation.tex <==
%\begin{table}[tb]
\caption{Ablation table to figure out the effectiveness of our training method in \refinemethod{}.
The results clearly show the success of \refinemethod{}.}
\label{tab:ablation_tab}
\centering
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{6}{c}{CIFAR-10} \\ \cmidrule{2-7}
% & $D_f(\downarrow)$ & $D_r(\uparrow)$ & $D_{ft}(\downarrow)$ & $D_{rt}(\uparrow)$ & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
% \midrule
% Original & 99.96 & 99.91 & 99.20 & 99.02 & 0.08 & 1.59\\
% \methodname & 1.90 & 98.49 & 2.04 & 99.63 & 98.29 & \underline{98.79}\\
% \methodname-2 & 0.00 & 99.92 & 0.00 & 99.06 & \textbf{99.96} & \textbf{99.53}\\
% \methodname-3 & 0.10 & 99.91 & 0.00 & 99.06 & \underline{99.90} & \textbf{99.53}\\
% \midrule
% Retrain & 0.00 & 99.91 & 0.00 & 99.00 & 99.95 & 99.50\\
% \bottomrule
% \end{tabular}

% \begin{tabular}{cccccc}
% \toprule
% \multicolumn{6}{c}{CIFAR-10$-RS$} \\ \cmidrule{1-6}
% $D_f(\downarrow)$ & $D_r(\uparrow)$ & $D_{ft}(\downarrow)$ & $D_{rt}(\uparrow)$ & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
% \midrule
% 99.98 & 99.89 & 99.40 & 98.92 & 0.04 & 1.19\\
% 74.54 & 99.74 & 72.90 & 98.76 & \underline{40.57} & \underline{42.53}\\
% 90.26 & 99.89 & 88.70 & 99.01 & 17.75 & 20.28\\
% 67.36 & 99.89 & 64.70 & 99.02 & \textbf{49.20} & \textbf{52.05}\\
%  \midrule
% 93.04 & 99.88 & 92.90 & 98.96 & 13.01 & 13.25\\   
% \bottomrule
% \end{tabular}
% }
\resizebox{\textwidth}{!}{
%{\scriptsize
\begin{tabular}{cccc}
\toprule
\multirow{2}{*}{$\mathcal{L}_{PCE}$} & \multirow{2}{*}{$\tau$}& \multicolumn{2}{c}{CIFAR-100} \\ \cmidrule{3-4}
&  & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
\midrule
%Original & & 98.42 & 98.10 & 93.30 & 93.12 & 3.11 & 12.50\\
% slice
& & 99.01 & 96.45\\
% mask learning
\checkmark & & \underline{99.04} & \underline{96.46} \\
% mask learning + threshold
\checkmark & \checkmark & \textbf{99.05} & \textbf{96.47}\\
%\midrule
%&Retrain & 0.00 & 98.48 & 0.00 & 93.16 & 99.23 & 96.46\\
\bottomrule
\end{tabular}

\begin{tabular}{cccc}
\toprule
\multicolumn{2}{c}{CIFAR-100$-RS$} \\ \cmidrule{1-2}
$HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
\midrule
%97.78 & 97.01 & 91.70 & 91.83 & 4.34 & 15.22\\
\textbf{98.30} & \textbf{95.70}\\
94.70 & 91.59\\
\underline{97.56} & \underline{95.11}\\
%\midrule
%71.34 & 97.17 & 71.20 & 91.90 & 44.26 & 43.86\\
\bottomrule
\end{tabular}
}
%}

% \resizebox{\textwidth}{!}{
% \begin{tabular}{cc|cccccc}
% \toprule
% \multirow{2}{*}{Mask learning} & \multirow{2}{*}{Threshold}& \multicolumn{6}{c}{CIFAR-100} \\ \cmidrule{3-8}
% &  & $D_f(\downarrow)$ & $D_r(\uparrow)$ & $D_{ft}(\downarrow)$ & $D_{rt}(\uparrow)$ & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
% \midrule
% %Original & & 98.42 & 98.10 & 93.30 & 93.12 & 3.11 & 12.50\\
% % slice
% & & 0.16 & 96.81 & 0.10 & 91.53 & 98.30 & 95.53\\
% % mask learning
% \checkmark & & 0.02 & 98.12 & 0.00 & 93.16 & \underline{99.04} & \underline{96.46} \\
% % mask learning + threshold
% \checkmark & \checkmark & 0.00 & 98.11 & 0.00 & 93.18 & \textbf{99.05} & \textbf{96.47}\\
% %\midrule
% %&Retrain & 0.00 & 98.48 & 0.00 & 93.16 & 99.23 & 96.46\\
% \bottomrule
% \end{tabular}

% \begin{tabular}{cccccc}
% \toprule
% \multicolumn{6}{c}{CIFAR-100$-RS$} \\ \cmidrule{1-6}
% $D_f(\downarrow)$ & $D_r(\uparrow)$ & $D_{ft}(\downarrow)$ & $D_{rt}(\uparrow)$ & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
% \midrule
% %97.78 & 97.01 & 91.70 & 91.83 & 4.34 & 15.22\\
% 0.44 & 91.18 & 0.30 & 86.47 & \underline{95.19} & \underline{92.61}\\
% 7.28 & 96.76 & 8.70 & 91.88 & 94.70 & 91.59\\
% 1.80 & 96.93 & 1.60 & 92.04 & \textbf{97.56} & \textbf{95.11}\\
% %\midrule
% %71.34 & 97.17 & 71.20 & 91.90 & 44.26 & 43.86\\
% \bottomrule
% \end{tabular}
% }

% \resizebox{\textwidth}{!}{
% \begin{tabular}{lcccccc}
% \toprule
% \multirow{2}{*}{Method} & \multicolumn{6}{c}{Tiny-ImageNet} \\ \cmidrule{2-7}
% & $D_f(\downarrow)$ & $D_r(\uparrow)$ & $D_{ft}(\downarrow)$ & $D_{rt}(\uparrow)$ & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
% \midrule
% Original & 96.72 & 96.47 & 90.30 & 90.24 & 6.34 & 17.52\\
% \methodname & 0.19 & 95.26 & 0.20 & 89.37 & \underline{97.48} & 94.30\\
% \methodname-2 & 0.02 & 96.53 & 0.20 & 90.50 & \textbf{98.22} & \underline{94.92}\\
% \methodname-3 & 0.00 & 96.50 & 0.00 & 90.50 & \textbf{98.22} & \textbf{95.01}\\
% \midrule
% Retrain & 0.00 & 95.24 & 0.00 & 90.81 & 97.56 & 95.18\\
% \bottomrule
% \end{tabular}

% \begin{tabular}{cccccc}
% \toprule
% \multicolumn{6}{c}{Tiny-ImageNet$-RS$} \\ \cmidrule{1-6}
% $D_f(\downarrow)$ & $D_r(\uparrow)$ & $D_{ft}(\downarrow)$ & $D_{rt}(\uparrow)$ & $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
% \midrule
% 99.98 & 99.89 & 99.40 & 98.92 & 0.04 & 1.19\\
% 0.32 & 91.88 & 0.20 & 86.03 & {95.62} & {92.40}\\
% 2.79 & 94.39 & 2.20 & 88.67 & \underline{95.78} & \underline{93.01}\\
% 1.44 & 94.59 & 0.90 & 88.66 & \textbf{96.53} & \textbf{93.59}\\
%  \midrule
% 71.15 & 94.16 & 69.30 & 88.74 & 44.17 & 45.62\\
% \bottomrule
% \end{tabular}
% }
%\end{table}



==> tab/tab_imagenet.tex <==
\begin{table}[tb]
\centering
\resizebox{0.9\columnwidth}{!}{
\begin{tabular}{lcc}
\toprule
\multirow{2}{*}{Method} & \multicolumn{2}{c}{ImageNet-1k} \\ \cmidrule{2-3}
& $HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
\midrule
Original & 21.41 & 30.86 \\
LAU~\cite{kim2023layer} & 80.25 & 76.61 \\
\textbf{\methodname{} (Ours)} & \underline{91.15} & \underline{88.34} \\
\textbf{\refinemethod{} (Ours)} & \textbf{91.78} & \textbf{88.98} \\
\bottomrule
\end{tabular}

\begin{tabular}{cc}
\toprule
\multicolumn{2}{c}{ImageNet-1k$-KR$} \\ \cmidrule{1-2}
$HM(\uparrow)$ & $HM_{\text{t}}(\uparrow)$ \\
\midrule
22.34 & 30.74 \\
22.34 & 30.74 \\
\textbf{91.71} & \textbf{88.98} \\
\underline{57.44} & \underline{61.31} \\
\bottomrule
\end{tabular}
}
\caption{Accuracy and RS using ViT.}
\label{tab:imagenet}
\end{table}
